Low-Latency Data Sharing in Erasure Multi-Way Relay Channels

We consider an erasure multi-way relay channel (EMWRC) in which several users share their data through a relay over erasure links. Assuming no feedback channel between the users and the relay, we first identify the challenges for designing a data sharing scheme over an EMWRC. Then, to overcome these challenges, we propose practical low-latency and low-complexity data sharing schemes based on fountain coding. Later, we introduce the notion of end-to-end erasure rate (EEER) and analytically derive it for the proposed schemes. EEER is then used to calculate the achievable rate and transmission overhead of the proposed schemes. Using EEER and computer simulations, the achievable rates and transmission overhead of our proposed schemes are compared with the ones of one-way relaying. This comparison implies that when the number of users and the channel erasure rates are not large, our proposed schemes outperform one-way relaying. We also find an upper bound on the achievable rates of EMWRC and observe that depending on the number of users and channel erasure rates, our proposed solutions can perform very close to this bound.

==> Cut_set.tex <==
Here, the common rate $R$ is upper bounded using the cut-set bound technique.
For each user (e.g. $n$), two cuts are considered: the cut assuming the relay and user $n$ as receivers of a multiple-access channel interested in decoding the rest of $N\!-\!1$ users, and the cut assuming the relay as the transmitter to user $n$. The sum-rate constraint is the dominant constraint in the multiple-access cut. Using similar arguments as \cite{Vishwanath_ITW_07}, it is easy to show that the sum-rate is bounded by $1\!-\!\epsilon_u^{N-1}$. The second cut is a simple single user erasure channel cut, which bounds the sum-rate by $1\!-\!\epsilon_d$. Therefore,
\begin{align}
(N-1)R&\le \min \{1-\epsilon_u^{N-1}, 1-\epsilon_d \}
\end{align}

==> EEER.tex <==
To study the performance of the three aformentioned schemes, we introduce a useful concept called end-to-end erasure rate (EEER). First, pairwise EEER is defined which is the erasure rate between a pair of users where one of them serves as the data source and the other one as destination. Having $N$ users in the systems results in $\frac{N(N-1)}{2}$ pairwise EEERs. Using pairwise EEER, the data transmission between the users within the pair is seen as a simple single-source single-destination erasure channel. Then, we define EEER referring to the worst (i.e. largest) pairwise EEER between a user pair over all possible cases. EEER is important to evaluate the achievable rate and fountain coding overhead of OWR, MPWR and OPPWR. In the following, we denote the pairwise EEER of user $i$ at user $j$ by $\epsilon_{i,j}$. According to our definition, EEER is defined as $\displaystyle{\epsilon_f = \max_{i,j} \epsilon_{i,j}}$.

\subsection{EEER Calculation for OWR}
Using OWR, a packet sent from user $i$ is received by user $j$ if it is not erased neither in the uplink nor in the downlink. Thus, defining $\bar{\epsilon}_{u_i} = 1 - \epsilon_{u_i}$ and $\bar{\epsilon}_{d_j} = 1 - \epsilon_{d_j}$, we have $\epsilon_{i,j} = 1 - \bar{\epsilon}_{u_i} \bar{\epsilon}_{d_j}.$ Now, EEER is
\begin{equation}
\epsilon_{f}^{\mathrm{OWR}} = \max_{i,j} \epsilon_{i,j} = 1 - \min_{i,j} \bar{\epsilon}_{u_i} \bar{\epsilon}_{d_j}.
\end{equation}
Note that the reconstruction process at the relay is not helpful when OWR is used since the relay receives the data of a specific user in only one uplink channel use. Further, for a symmetric EMRWC where for all $i$, $\epsilon_{u_i} = \epsilon_u$ and $\epsilon_{d_i} = \epsilon_d$, pairwise EEERs are all equal for any pair of users. Note that since in OWR, the data packet of each users is transmitted to the relay in only one uplink slot, reconstruction cannot improve its performance.


\subsection{EEER Calculation for MPWR}
For MPWR, the relay receives the data of each user (except the first and last user) in two uplink time slots. Thus, it may be able to employ data reconstruction for $u_2$ to $u_{N - 1}$ in order to retrieve their data if it is erased in only one uplink transmissions. In the following, we study EEER for both cases when the relay does not perform data reconstruction and when it does.

\textit{MPWR without Reconstruction:} First, we study $\epsilon_{i,1}$, the pairwise EEER of $u_i$, $i=2,\ldots,N$, at $u_1$. Then we extend the analysis to other users. For decoding at $u_1$, let us call the probability of finding $x_i$ at $i$th or $(i+1)$th rows of $\textbf{A}_1$ by $P_1^1(i)$ and $P_2^1(i)$ respectively.

First, we calculate $P_1^1(i)$. Notice that $P_1^1(1) = 1$ since $x_1$ is always known at $u_1$. For $i > 1$, $x_i$ is found in row $i$ when this row is not erased in the downlink phase and : (i) No erasure has happened in row $i$ during the uplink phase and the value of $x_{i-1}$ has been found from row $i - 1$ or (ii) In the $i$th row, $x_{i-1}$ was erased in the uplink phase, while $x_i$ has been perfectly received (only $x_i$ exists in this row). Hence,
\begin{equation}\label{Eq P_1}
P_1^1(i) = \bar{\epsilon}_{d_1} (\bar{\epsilon}_{u_i} \bar{\epsilon}_{u_{i - 1}} P_1(i-1) + \bar{\epsilon}_{u_{i}} \epsilon_{u_{i-1}}).
\end{equation}
Having $P_1^1(1) = 1$, by solving the above recursive equation for $i = 2,\ldots,N$, all $P_1^1(i)$'s are found.

Now, we calculate $P_2^1(i)$. Since $x_N$ appears just once in (\ref{Eq linear system}) when MPWR is used, $P_2^1(N) = 0$. Also $P_2^1(1) = 1$. By a logic similar to the one used for the calculation of $P_1^1(i)$, for $i=2,\ldots,N-1$, we have
\begin{equation}
P_2^1(i) = \bar{\epsilon}_{d_1} (\bar{\epsilon}_{u_i} \bar{\epsilon}_{u_{i + 1}} P_2(i+1) + \bar{\epsilon}_{u_i} \epsilon_{u_{i+1}}).
\end{equation}

Now, to complete the pairwise EEER calculation, we just need to find $P_c^1(i)$ representing the probability of finding $x_i$ at $u_1$ in both $i$ and $(i +1)$th equations. Here, $x_i$ can be retrieved from both $i$th and $(i+1)$th rows if none of these rows is erased in the downlink and $x_i$ does exist in both rows. Also, one of these situations should happen: (i) $x_{i-1}$ in row $i$ and $x_{i+1}$ in row $i+1$ are both erased in the uplink phase, (ii) Either $x_{i-1}$ or $x_{i+1}$ is erased in the uplink phase and the other one was found before solving the corresponding equation, (iii) Nothing is erased in the uplink phase and $x_{i-1}$ and $x_{i+1}$ have been previously found. Thus, for $i=2,\ldots,N$, we have
\begin{align}\label{Eq P_c}
P_c^1(i) \! \!= \! \bar{\epsilon}_{d_1}^2  \bar{\epsilon}_{u_i}^2 \! \Big[\epsilon_{u_{i-1}} \epsilon_{u_{i+1}}  \! + \! \epsilon_{u_{i+1}} \bar{\epsilon}_{u_{i-1}} P_1^1(i\!-\!1\!) \!+ \epsilon_{u_{i-1}} \bar{\epsilon}_{u_{i+1}} P_2^1(i\!+\!1\!) \!+\! \bar{\epsilon}_{u_{i+1}} \bar{\epsilon}_{u_{i+1}} P_1^1(i\!-\! 1) P_2^1(i \!+\!1\!)\Big].
\end{align}
%Notice that in (\ref{Eq P_c}), for $n = N$, we should set $P_2(n + 1) = P_2(1) = 1$. This is because $x_1$ appears with $x_n$ for the second time and is always known at $u_1$.

Now, the probability of finding $x_i$ at $u_1$ is
\begin{equation}
P^1(i) = P_1^1(i) + P_2^1(i) - P_c^1(i)
\end{equation}
and $\epsilon_{i,1} = 1 - P^1(i)$.

Let us derive the probability of finding $x_i$ at user $j$, called $P^j(i)$. Since $x_j$ is known at user $j$, finding the values of $x_{j-1},x_{j-2},\ldots,x_1$ can be casted into finding $x_2,x_3,\ldots,x_j$ at $u_1$ when there are only $j$ users in the system trying to exchange their data. Thus, for $i=1,2,\ldots,j-1$, $P^j(i) = P^1(j - i +1)$ where $P^1(\cdot)$ is calculated when there are $j$ users in the system. Similarly, for $i = j+1,j+2,\ldots,N$, we have $P^j(i) = P^1(i - j + 1)$ when only $N - j + 1$ users exchange their data. Hence, $\epsilon_{i,j}$ is derived. Similar to OWR, $\epsilon_{f}^{\mathrm{MPWR}} = \displaystyle{\max_{i,j} \epsilon_{i,j}}$. Furthermore, the average erasure rate that each user experiences is
\begin{equation} \label{Eq Average erasure MPWR}
\epsilon_{\mathrm{ave}}^{MPWR} = 1 - \frac{\displaystyle{\sum_{j=1}^N \sum_{i=1,i \neq j}^N P^j(i)}}{N (N -1)}.
\end{equation}
The importance of $\epsilon_{\mathrm{ave}}^{MPWR}$ is later discussed in Subsection \ref{Subsection Numerical Examples}.


\rem \label{Remark MPWR} Assume a symmetric EMWRC where $\epsilon_{u_i} = \epsilon_{u}$ and $\epsilon_{d_i} = \epsilon_{d}$ for all $i$. In this case, unlike OWR, pairwise EEERs are not necessarily equal at different users when MPWR is used. Further, it can be shown that
\begin{equation}
\min_{j,i} P^j(i) = P^1(N) = P^N(1).
\end{equation}
Thus, $\epsilon_f^{\mathrm{MPWR}} = \displaystyle{\max_{i,j} \epsilon_{i,j} = 1 - P^1(N)}$.

\textit{MPWR with Reconstruction:} Reconstruction at the relay is performed on $\textbf{A}_r$ and gives $\tilde{\textbf{A}}$. Its purpose is to reduce the uplink erasure rate without affecting the downlink. In the following, we find the equivalent uplink erasure rate when MPWR along with relay reconstruction is used. The equivalent uplink erasure probability of $x_i$ in $j$th pairwise transmission is the probability of not being able to retrieve it at $j$th equation even after reconstruction at the relay. Notice that $x_i$ appears in $(i-1)$th and $i$th equations of $\textbf{A}$. Thus, $j \in \{i-1 ,i \}$.

First of all, if $x_1$ or $x_N$ is erased in its associated transmission, it never can be retrieved since these data packets appear in only one row of $\textbf{A}$. Now, assume that $x_i$, $2 \leq i \leq N - 1$, is erased in $(i - 1)$th equation. To find $x_i$ from the rest of equations, one of these cases should happen: i) $x_{i+1}$ is erased in $i$th equation while $x_i$ exists there, ii) Both $x_i$ and $x_{i+1}$ exist in $i$th equation, and only $x_{i+1}$ is received by the relay in $(i+1)$th equation .... This continues until the case where all $x_i$'s in the $i$th to $(N-2)$th equations exist and $x_N$ is erased from the $(N-1)$th row of $\textbf{A}$ while $x_{N-1}$ exists. Thus, the probability of retrieving $x_i$ in the $(i-1)$th row of $\textbf{A}_r$ when it has been originally erased in the uplink transmission is
\begin{align}
P_{c}^{i,i-1}  \! = \! \bar{\epsilon}_{u_i} \epsilon_{u_{i+1}} \! + \! \bar{\epsilon}_{u_i} \bar{\epsilon}^2_{u_{i+1}} \epsilon_{u_{i+2}} \! + \! \ldots + \bar{\epsilon}_{u_i} \bar{\epsilon}^2_{u_{i+1}} \cdots \bar{\epsilon}_{u_{N - 1}}^2 \epsilon_{u_N}  = \bar{\epsilon}_{u_i} \sum_{j=i+1}^{N} \{ \epsilon_{u_j} \prod_{k=i+1}^{j - 1} \bar{\epsilon}_{u_k}^2 \}.
\end{align}
Having $P_{c}^{i,i-1}$, the equivalent uplink erasure rate of $x_{i}$ in $(i - 1)$th equation is
\begin{equation}
\epsilon_{u}^{i,i-1} = \epsilon_{u_{i}} ( 1 - P_{c}^{i,i-1}).
\end{equation}

Now, assume that $x_i$ is erased in $i$th equation. It can be found if: i) $x_i$ appears in $(i-1)$th equation while $x_{i-1}$ is erased, ii) Both $x_i$ and $x_{i-1}$ appear in $(i - 1)$th equation and only $x_{i - 1}$ is received by relay in $(i - 2)$th equation. \ldots The last possible situation is when $x_1$ is erased in the first equation while $x_2$ exists and none of $x_j$'s in the second to $(i - 1)$th equations is erased. Thus, the probability of erasure correction for $x_i$ at equation $i$ is
\begin{align}
P_{c}^{i,i}  \! = \! \bar{\epsilon}_{u_i} \epsilon_{u_{i-1}} \! + \! \bar{\epsilon}_{u_i} \bar{\epsilon}^2_{u_{i-1}} \epsilon_{u_{i-2}} \! + \! \ldots + \bar{\epsilon}_{u_i} \bar{\epsilon}^2_{u_{i-1}} \cdots \bar{\epsilon}_{u_{2}}^2 \epsilon_{u_1}  = \bar{\epsilon}_{u_i} \sum_{j=1}^{i-1} \{ \epsilon_{u_j} \prod_{k=j+1}^{i - 1} \bar{\epsilon}_{u_k}^2 \}.
\end{align}
Similarly, the equivalent uplink erasure rate of $u_i$ when it experiences erasure in $i$th uplink transmission is
\begin{equation}
\epsilon_{u}^{i,i} = \epsilon_{u_{i}} ( 1 - P_{c}^{i,i}).
\end{equation}
Notice that $P_c^{1,1} = P_c^{N,N - 1} = 0$. To apply the effect of reconstruction on EEER calculation, we should properly replace $\epsilon_{u_i}$ with either $\epsilon_{u}^{i,i-1}$ or $\epsilon_{u}^{i,i}$. In other words, $x_i$ experiences erasure in the $i$th row of $\textbf{A}_1$ with $\epsilon_{u}^{i,i-1}$ and with $\epsilon_{u}^{i,i}$ in the $(i + 1)$th row.

\rem For a symmetric EMWRC with MPWR, it can be shown that by increasing $N$, by averaging $P_{c}^{i,i-1}$ and $P_{c}^{i,i}$ over all $i$'s, we have
\begin{align}
E(P_c^{i,i-1}) \approx  \frac{\bar{\epsilon_u}}{1 + \bar{\epsilon_u}},\\
E(P_c^{i,i}) \approx  \frac{\bar{\epsilon_u}}{1 + \bar{\epsilon_u}},
\end{align}
where $E(\cdot)$ stands for the expected value. As a consequence, both $\epsilon_{u}^{i,i-1}$ and $\epsilon_{u}^{i,i}$ approach $\frac{\epsilon_u}{2 - \epsilon_u}$.

\subsection{EEER Calculation for OPPWR}
\textit{OPPWR without Reconstruction:} Consider one round of communication for OPPWR which consists of $N$ pairwise user transmissions. Since for OPPWR, $\textbf{A}$ is a circulant matrix, without loss of generality, we find $\epsilon_{i,1}$ for $i = 2,3,\ldots,N$. Other pairwise EEERs are similarly found by proper circulation of $\epsilon_{i,1}$.


Having $x_1$ (the first row of $\textbf{A}_1$ in (\ref{Eq A_1})), $u_1$ can find $x_i$ either in row $i$  or $i + 1$ of (\ref{Eq linear system}) for $i = 2,3,\ldots,N$. Let us denote the probability of finding $x_i$ in row $i$ and $i + 1$ by $P_1(i)$ and $P_2(i)$ respectively. Thus, the probability of retrieving $x_i$ in $u_1$, $P(i)$, is
\begin{equation} \label{Pn OOPW}
P(i) = P_1(i) + P_2(i) - P_c(i)
\end{equation}
where $P_c(i)$ is the probability of being able to retrieve $x_i$ in both $i$th and $(i+1)$th rows of $\textbf{A}_1$.

$P_1(i)$ is found similar to (\ref{Eq P_1}). Further, due to the cyclic structure of $\textbf{A}$, it can be shown that $P_2(i) = P_1(N - i + 2)$ for $i=2,3,\ldots,N$. Derivation of $P_c(i)$ is also similar to (\ref{Eq P_c}). To calculate $P_c(i)$ in (\ref{Eq P_c}), we should substitute $P_2(i + 1)$ by $P_2(1) = 1$ when $i = N$. This is because $x_1$ appears with $x_N$ for the second time and is always known at $u_1$. Having all terms in (\ref{Pn OOPW}), $\epsilon_{i,1} = 1 - P(i)$. Further, using the circulant structure of $\textbf{A}$, it can be shown that $\epsilon_{i,j} = \epsilon_{i - j + 1,1}$. Having the pairwise EEERs, $\epsilon_f^{\mathrm{OPPWR}} = \displaystyle{\max_{i,j} \epsilon_{i,j}}$ and users' average erasure rate, $\epsilon_{\mathrm{ave}}^{OPPWR}$, is simply calculated similar to (\ref{Eq Average erasure MPWR}).

\rem \label{Remark OPPWR} For a symmetric EMWRC, EEERs can be different for different users when OPPWR is used. In this case, it can be shown that $\epsilon_f^{\mathrm{OPPWR}} = \epsilon_{\lfloor N/2 \rfloor + 1,1}$.


\textit{OPPWR with Reconstruction:}
Similar to MPWR, we calculate $\epsilon_{u}^{i,i-1}$ and $\epsilon_{u}^{i,i}$ to derive the uplink equivalent erasure rate. With a similar logic, it can be shown that for OPW
\begin{align}
P_c^{i,i-1} \! &= \! \bar{\epsilon}_{u_i} \epsilon_{u_{i+1}} \! + \! \bar{\epsilon}_{u_i} \bar{\epsilon}^2_{u_{i+1}} \epsilon_{u_{i+2}} \! + \! \ldots + \bar{\epsilon}_{u_i} \bar{\epsilon}^2_{u_{i+1}} \cdots \bar{\epsilon}_{u_{N}}^2 \bar{\epsilon}_{u_{1}}^2 \cdots \bar{\epsilon}_{u_{i-2}}^2 \epsilon_{u_{i-1}} \\
& = \bar{\epsilon}_{u_i} \sum_{j=i}^{N + i - 2} \{ \epsilon_{u_{m(j) + 1}} \prod_{k=i}^{j - 1} \bar{\epsilon}_{u_{m(k) + 1}}^2 \}.
\end{align}
and
\begin{align}
P_c^{i,i} \! &= \! \bar{\epsilon}_{u_i} \epsilon_{u_{i-1}} \! + \! \bar{\epsilon}_{u_i} \bar{\epsilon}^2_{u_{i-1}} \epsilon_{u_{i-2}} \! + \! \ldots + \bar{\epsilon}_{u_i} \bar{\epsilon}^2_{u_{i-1}} \cdots \bar{\epsilon}_{u_{1}}^2 \bar{\epsilon}_{u_{N}}^2 \cdots \bar{\epsilon}_{u_{i+2}}^2 \epsilon_{u_{i+1}} \\
&= \bar{\epsilon}_{u_i} \sum_{j=1}^{N - 1} \{ \epsilon_{u_{m(i - j)}} \prod_{k=1}^{j - 1} \bar{\epsilon}_{u_{m(i - k)}}^2 \}
\end{align}
where $m(\cdot)$ represents modulo-$N$ operation. Other stages of EEER calculation are similar to what described for MPWR.

\rem For a symmetric EMWRC with OPPWR, it can be shown that for all $i$, $P_c^{i,i-1} = P_c^{i,i} = P_c$. Further, by increasing $N$,
\begin{equation}
P_c \approx \frac{\bar{\epsilon_u}}{1 + \bar{\epsilon_u}}
\end{equation}
where $\bar{\epsilon_u} = 1 - \epsilon_u$. As a consequence, the equivalent uplink erasure probability for all users are equal. We name it by $\epsilon_u'$ and $\epsilon_u' \approx \frac{\epsilon_u}{2 - \epsilon_u}.$


\subsection{Numerical Examples} \label{Subsection Numerical Examples}
Here, we present some numerical examples to appreciate the role of reconstruction at the relay. Further, we discuss how the EEER can be decrease by modifying the users' transmission scheduling and employ a shuffled transmission schedule for users. The following cases are for a symmetric EMWRC with uplink and downlink erasure probabilities $\epsilon_u$ and $\epsilon_d$ respectively.

Figure \ref{Fig EEER for MPWR} depicts EEER (maximum pairwise EEER), average pairwise EEER and the minimum pairwise EEER among the users when MPWR is used. As seen, there is a significantly large gap between EEER and average pairwise EEER. Similar results are presented in Figure \ref{Fig EEER for OPPWR} when OPPWR is used. Having such a large variance between pairwise EEERs noticeably limits the achievable rate of the system. Please note that for OWR, all pairwise EEERs are equal, thus, numerical results are omitted here.

\begin{figure}[h!]
\centering
\includegraphics[scale=.6]{Rateless/MPW.ps}
\caption{EEER, average pairwise EEER and minimum EEER for MPWR.} \label{Fig EEER for MPWR}
\end{figure}


\begin{figure}[h!]
\centering
\includegraphics[scale=.6]{Rateless/OPPW.ps}
\caption{EEER, average pairwise EEER and minimum EEER for OPPWR.} \label{Fig EEER for OPPWR}
\end{figure}


To improve the system's achievable rate, it is desired to narrow the gap between EEER and average pairwise EEER. For this purpose, we suggest using a shuffled (random) transmission scheduling. In this approach, all users have psuedorandom number generators with the same initial seeds. Thus, the output of number generators are equal at all users. For each round of communication, psuedorandom number generators give a random permutation of numbers from 1 to $N$. We denote this psuedorandom sequence by $\{S_1,S_2,\ldots,S_N \}$. This random sequence specifies the order of transmission by users. For our proposed pairwise schemes, in the first uplink transmission, user $S_1$ and user $S_2$ transmit, in the second uplink transmission, user $S_2$ and user $S_3$ transmit and so on. For OPPWR, user $S_N$ and user $S_1$ also transmit together in the last uplink slot.

In the abovementioned shuffled scheduling, $i$th row of $\textbf{A}$ is assigned to the pairwise transmission of $u_{S_i}$ and $u_{S_{i + 1}}$ for each round of communication. Note that $u_{S_i}$ and $u_{S_{i + 1}}$ can be any arbitrary two users from $u_1$ to $u_N$ in each round. Thus, by doing shuffled scheduling over large number of communication rounds, we expect EEER and minimum pairwise EEER to converge to the average pairwise EEER. As a consequence, shuffled transmission scheduling significantly evens out the pairwise erasure rates resulting in a lower overall EEER.

Effect of the reconstruction on the equivalent uplink erasure probability is presented in Figure~\ref{Fig Equivalent Uplink erasure for MPWR} and Figure~\ref{Fig Equivalent Uplink erasure for OPPWR} for MPWR and OPPWR, respectively. In these figures, the average equivalent uplink erasure probability over all users is depicted versus the uplink erasure probability and the number of users. As seen, for small $N$, reconstruction is not much helpful when MPWR is used. For instance, if $N = 2$, reconstruction does not improve the performance at all since the data of each user (here two users) exist in only one uplink transmission. Hence, there is no redundancy for retrieving the users' data from other uplink transmissions if it is erased. On the other hand, reconstruction causes the best improvement in terms of erasure rate for OPPWR when $N = 2$. This is due to the repetitive transmission of users' data (each user data packet in sent twice). As number of users increases, performance improvement by reconstruction increases for MPWR while it decreases for OPPWR. However, generally speaking, reconstruction at the relay has a more significant improvement for OPPWR.

\begin{figure}[h!]
\centering
\includegraphics[scale=.6]{Rateless/MPW_Reconst.ps}
\caption{Equivalent Uplink erasure probability for MPWR.} \label{Fig Equivalent Uplink erasure for MPWR}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[scale=.6]{Rateless/OPPW_Reconst.ps}
\caption{Equivalent Uplink erasure for probability OPPWR.} \label{Fig Equivalent Uplink erasure for OPPWR}
\end{figure}

                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          

==> Introduction_Long.tex <==
The concept of two-way communication was first investigated by Shannon \cite{shannon_twoway} and later, multi-way channels were considered. A summary of the early studies on multi-way channels is presented by Meulen in \cite{Mulen_Multi_way_IT1977}. Further, relay channels have been a prominent topic in communications \cite{Meulen_Relay,Cover_Relay_TIT} since their early stage. However, the combination of two-way channels and relay channels appeared many years later in \cite{Rankov_Two_way_Asilomar2005} and \cite{Popovski_TwoWay_ICC2006} in the form of two-way relay channels (TWRCs). Then, Gunduz \textit{et al.} extended TWRCs and introduced multi-way relay channels (MWRCs) \cite{Gunduz_Multi_way_ISIT2009}.

In an MWRC, multiple users want to (fully) exchange their data with each other. The users do not have any direct link to one another and consequently a relay is used to enable the communication between them. Some practical examples of multi-way relaying are file sharing between several devices or conference calls in a cellular network.

MWRCs have been studied for Gaussian \cite{Gunduz_Multi_way_ISIT2009,Ong_FDF_Gaussian_ISIT2010} and binary symmetric \cite{Ong_FDF_CommLetter_2010} channels when the channel information is known at the relay as well as users. Hence, they can apply appropriate channel coding techniques accordingly. However, this information may not be always known, e.g. when the links between the users and relay are time-varying. In this situation, channel coding fails to provide error-free communication. From the viewpoint of higher network layers, this is seen as an erasure channel where the data is received either perfectly or completely erased. Our present work focuses on the low-latency communication schemes applicable to multi-way relay erasure channels (MWRECs). In particular, we consider the ``binary'' erasure channel\footnote{Our analysis can be readily extended to larger alphabet sizes.}.

Fountain coding is a strong candidate to combat data erasure and is known to be near-optimal for every erasure channel \cite{MacKay_book_03}. The notion of fountain coding for wireless relay networks has been originally proposed in \cite{Castura_Rateless_ISIT} where one source sends its data through one or more relays to a destination. Later, fountain coding was applied to different relay networking setups, e.g \cite{Puducheri_DLT_IT2007,Gummadi_RelayFountain_ITW2008}. The main point distinguishing rateless relaying in an MWREC with the current studied rateless relaying schemes is the existence of the side information in each user (i.e. each user knows its own data). Further, applying fountain coding over MWRECs has two other important challenges. First, it is undesirable to perform fountain decoding and encoding at the relay owing to its inordinate delay. Thus, fountain encoding and decoding should be all performed at the users. This necessitates the design of low-latency fountain schemes. Also, the fountain scheme should be scalable for any number of users.

In this work, we propose two fountain schemes, namely minimal pairwise (MPW) and one-level protected pairwise (OPPW). In these schemes, each user encodes its own data with a fountain code. To make the data of any arbitrary user decodable from other users' data, we employ a pairwise transmission strategy employing network coding to enhance spectral efficiency. MPW is basically similar to the approach taken in \cite{Ong_FDF_CommLetter_2010} where two users simultaneously transmit in the uplink. OPPW is a variant of MPW benefiting from a higher erasure protection at the cost of an extra uplink and downlink transmission. We show that MPW has in fact the minimum number of users' transmissions and lowest latency among all possible pairwise schemes. Both approaches are easily applicable to an MWREC with any number of users. Further, the fountain encoders at the users are synchronized to ease the system implementation. The details of these schemes are discussed in Section \ref{Section System model}.


After developing MPW and OPPW, we employ them in the situation where the relay is memoryless and does not perform any operation on the received data. Then, we extend our approaches to the case when the relay has a limited buffer size and is capable of performing simple operations. To this end, we propose a data reconstruction strategy for the relay in order to compensate the data erasure in the uplink. Also, EEP is analytically derived for both MPW and OPPW.


In a fountain scheme, to assure that the data of one user are decodable at another user, a certain number of data bits (packets) has to be perfectly received by the user. This number is mainly determined by the data erasure probability at the receiver. In our problem, the data erasure comprises channel erasure effect as well as the possibility of not being able to decode the users' data from the relay transmitted message. To this end, we first introduce the notion of \emph{equivalent erasure probability} (EEP). Here, EEP is the probability of not being able to retrieve the transmitted packet of one user in another user. EEP is used to evaluate the performance of our developed fountain schemes.

Using EEP, we first compare the achievable rate of MPW and OPPW with the cut-set upper bound and the achievable rate of one-way (OW) relaying scheme. As seen in Section \ref{Section Performance}, when no erasure happens (ideal channel), MPW achieves the cut-set bound. By increasing the channel erasure probability and for small number of users, $N$, MPW still achieves a higher rate than OPPW and OW and gets close to the cut-set bound. By increasing $N$, OPPW outperforms the other two methods. For large $N$, OW achieves higher rates than MPW and OPPW. %For small channel erasure probabilities, our schemes show better performance over one-way relaying in a larger range of $N$.

We then evaluate the performance of our proposed schemes in terms of the average and maximum overhead required for decoding at the users. Average overhead, $O_{\mathrm{av}}$, is the average overhead per user required for fountain decoding at another user. Maximum overhead, $O_{\mathrm{max}}$, represents the overhead needed to make sure that all users have successfully decoded the data of others. Notice that the maximum overhead is a measure of maximum delay in the system. Comparing the analytical results (based on EEP) for $O_{\mathrm{av}}$ and $O_{\mathrm{max}}$ with the simulation results verifies the analysis accuracy and usefulness of EEP. The performance trend for $O_{\mathrm{av}}$ and $O_{\mathrm{max}}$ is similar to the achievable rate.

%Our analysis reveals that depending on the number of users, and erasure probabilities, the strategy will change. More specifically, for small $N$, we select MPW; for moderate $N$, OPPW is the best choice; and for large $N$ values, OW outperforms the rest. 
